Feature-Realistic Neural Fusion for Real-Time, Open Set Scene Understanding

General scene understanding for robotics requires flexible semantic representation, so that novel objects and structures which may not have been known at training time can be identified, segmented and grouped. We present an algorithm which fuses general learned features from a standard pre-trained network into a highly efficient 3D geometric neural field representation during real-time SLAM. The fused 3D feature maps inherit the coherence of the neural field's geometry representation. This means that tiny amounts of human labelling interacting at runtime enable objects or even parts of objects to be robustly and accurately segmented in an open set manner.

==> symbols.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Original content of newcom.tex starts here
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\unitlength=1mm

\newcommand{\TODO}[1]{~\\ \textbf{TODO:} #1}
\newcommand{\ignore}[1]{}

\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beas}{\begin{eqnarray*}}
\newcommand{\eeas}{\end{eqnarray*}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bfig}{\begin{figure}}
\newcommand{\efig}{\end{figure}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\bpic}{\begin{picture}}
\newcommand{\epic}{\end{picture}}
\newcommand{\btabular}{\begin{tabular}}
\newcommand{\etabular}{\end{tabular}}
\newcommand{\btable}{\begin{table}}
\newcommand{\etable}{\end{table}}

% Black and white \bs and \es
%\newcommand{\bs}[1]{\begin{slide}{}{\tiny #1} \\
%                    \rule[6mm]{170mm}{0.7mm}}
%\newcommand{\es}{\vfill
%                 \rule[-6mm]{170mm}{0.7mm} \\
%                 {\tiny
%		  \hfill S-\theslide}
%                 \end{slide}}
%\newcommand{\Ltitle}[1]{\bc {\Large\textbf \vspace{-15mm} #1} \ec}
%\newcommand{\ltitle}[1]{\bc {\large\textbf \vspace{-15mm} #1} \ec}

% Colour versions of \bs and \es
%\newcommand{\bs}[1]{\begin{slide}{}\redw{{\tiny #1}} \\
%                    \rule[6mm]{170mm}{0.7mm}}

\newcommand{\es}{\vfill
                 \rule[-6mm]{170mm}{0.7mm} \\
                 \redw{{\tiny
		  \hfill S-\theslide}}
                 \end{slide}}
\newcommand{\Ltitle}[1]{\bc {\Large\textbf \vspace{-15mm} #1} \ec}
\newcommand{\ltitle}[1]{\bc {\large\textbf \vspace{-15mm} #1} \ec}

\newcommand{\ruleoff}{\mbox{\\\rule{\columnwidth}{0.1mm}}}

% Originally \newcommand{\dsp}{\setlength{\baselineskip}{22truept}}
%\newcommand{\dsp}{\setlength{\baselineskip}{21truept}}
\newcommand{\matxx}[1]{{\mathtt #1}}
\newcommand{\vecXX}[1]{{\mathbf {#1}}}
\newcommand{\vecYY}[1]{{\boldsymbol {#1}}}

\newcommand{\icap}[1]{{\caption{\em #1}}}

\def \nor {\normalsize}

\newcommand{\argmin}{\operatornamewithlimits{arg\ min}}
\newcommand{\argmax}{\operatornamewithlimits{arg\ max}}
\newcommand{\maxarg}{\operatornamewithlimits{\ max}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Original content of symbols.tex starts here
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def \crossprod {\times}
\def \dotprod {\bullet}
\providecommand{\etal}{{\em et~al.}}
\def \grad {\mbox{\boldmath $\nabla$}}
\def \gradE {\mbox{{\boldmath $\nabla$}} E}
\def \half {\frac{1}{2}}
\def \matxTx {[{\texttt t}_\times]}
\def \matxminusTx {[{\texttt -t}_\times]}
\def \trans {{\top}}
\def \cosec {\mbox{cosec}}

\def \ahat {{\hat{a}}}
\def \bhat {{\hat{b}}}
\def \chat {{\hat{c}}}
\def \dhat {{\hat{d}}}
\def \ehat {{\hat{e}}}
\def \fhat {{\hat{f}}}
\def \ghat {{\hat{g}}}
\def \hhat {{\hat{h}}}
\def \ihat {{\hat{i}}}
\def \jhat {{\hat{j}}}
\def \khat {{\hat{k}}}
\def \lhat {{\hat{l}}}
\def \mhat {{\hat{m}}}
\def \nhat {{\hat{n}}}
\def \ohat {{\hat{o}}}
\def \phat {{\hat{p}}}
\def \qhat {{\hat{q}}}
\def \rhat {{\hat{r}}}
\def \shat {{\hat{s}}}
\def \that {{\hat{t}}}
\def \uhat {{\hat{u}}}
\def \vhat {{\hat{v}}}
\def \what {{\hat{w}}}
\def \xhat {{\hat{x}}}
\def \yhat {{\hat{y}}}
\def \zhat {{\hat{z}}}

\def \Ahat {{\hat{A}}}
\def \Bhat {{\hat{B}}}
\def \Chat {{\hat{C}}}
\def \Dhat {{\hat{D}}}
\def \Ehat {{\hat{E}}}
\def \Fhat {{\hat{F}}}
\def \Ghat {{\hat{G}}}
\def \Hhat {{\hat{H}}}
\def \Ihat {{\hat{I}}}
\def \Jhat {{\hat{J}}}
\def \Khat {{\hat{K}}}
\def \Lhat {{\hat{L}}}
\def \Mhat {{\hat{M}}}
\def \Nhat {{\Hat{N}}}
\def \Ohat {{\hat{O}}}
\def \Phat {{\hat{P}}}
\def \Qhat {{\hat{Q}}}
\def \Rhat {{\hat{R}}}
\def \Shat {{\hat{S}}}
\def \That {{\hat{T}}}
\def \Uhat {{\hat{U}}}
\def \Vhat {{\hat{V}}}
\def \What {{\hat{W}}}
\def \Xhat {{\hat{X}}}
\def \Yhat {{\hat{Y}}}
\def \Zhat {{\hat{Z}}}

\def \abar {{\bar{a}}}
\def \bbar {{\bar{b}}}
\def \cbar {{\bar{c}}}
\def \dbar {{\bar{d}}}
\def \ebar {{\bar{e}}}
\def \fbar {{\bar{f}}}
\def \gbar {{\bar{g}}}
\def \hbar {{\bar{h}}}
\def \ibar {{\bar{i}}}
\def \jbar {{\bar{j}}}
\def \kbar {{\bar{k}}}
\def \lbar {{\bar{l}}}
\def \mbar {{\bar{m}}}
\def \nbar {{\bar{n}}}
\def \obar {{\bar{o}}}
\def \pbar {{\bar{p}}}
\def \qbar {{\bar{q}}}
\def \rbar {{\bar{r}}}
\def \sbar {{\bar{s}}}
\def \tbar {{\bar{t}}}
\def \ubar {{\bar{u}}}
\def \vbar {{\bar{v}}}
\def \wbar {{\bar{w}}}
\def \xbar {{\bar{x}}}
\def \ybar {{\bar{y}}}
\def \zbar {{\bar{z}}}

\def \vecnought {{\vecXX{0}}}
\def \veca {{\vecXX{a}}}
\def \vecb {{\vecXX{b}}}
\def \vecc {{\vecXX{c}}}
\def \vecd {{\vecXX{d}}}
\def \vece {{\vecXX{e}}}
\def \vecf {{\vecXX{f}}}
\def \vecg {{\vecXX{g}}}
\def \vech {{\vecXX{h}}}
\def \veci {{\vecXX{i}}}
\def \vecj {{\vecXX{j}}}
\def \veck {{\vecXX{k}}}
\def \vecl {{\vecXX{l}}}
\def \vecm {{\vecXX{m}}}
\def \vecn {{\vecXX{n}}}
\def \veco {{\vecXX{o}}}
\def \vecp {{\vecXX{p}}}
\def \vecq {{\vecXX{q}}}
\def \vecr {{\vecXX{r}}}
\def \vecs {{\vecXX{s}}}
\def \vect {{\vecXX{t}}}
\def \vecu {{\vecXX{u}}}
\def \vecv {{\vecXX{v}}}
\def \vecw {{\vecXX{w}}}
\def \vecx {{\vecXX{x}}}
\def \vecy {{\vecXX{y}}}
\def \vecz {{\vecXX{z}}}

\def \vecA {{\vecXX{A}}}
\def \vecB {{\vecXX{B}}}
\def \vecC {{\vecXX{C}}}
\def \vecD {{\vecXX{D}}}
\def \vecE {{\vecXX{E}}}
\def \vecF {{\vecXX{F}}}
\def \vecG {{\vecXX{G}}}
\def \vecH {{\vecXX{H}}}
\def \vecI {{\vecXX{I}}}
\def \vecJ {{\vecXX{J}}}
\def \vecK {{\vecXX{K}}}
\def \vecL {{\vecXX{L}}}
\def \vecM {{\vecXX{M}}}
\def \vecN {{\vecXX{N}}}
\def \vecO {{\vecXX{O}}}
\def \vecP {{\vecXX{P}}}
\def \vecQ {{\vecXX{Q}}}
\def \vecR {{\vecXX{R}}}
\def \vecS {{\vecXX{S}}}
\def \vecT {{\vecXX{T}}}
\def \vecU {{\vecXX{U}}}
\def \vecV {{\vecXX{V}}}
\def \vecW {{\vecXX{W}}}
\def \vecX {{\vecXX{X}}}
\def \vecY {{\vecXX{Y}}}
\def \vecZ {{\vecXX{Z}}}

\def \vecalpha {{\vecYY{\alpha}}}
\def \vecbeta  {{\vecYY{\beta}}}
\def \vecgamma {{\vecYY{\gamma}}}
\def \veceta   {{\vecYY{\eta}}}
\def \vecmu    {{\vecYY{\mu}}}
\def \vecnu    {{\vecYY{\nu}}}
\def \vecxi    {{\vecYY{\xi}}}
\def \vecomega {{\vecYY{\omega}}}

\def \vecAlpha {{\vecYY{\Alpha}}}
\def \vecOmega {{\vecYY{\Omega}}}

\def \Abar {{\bar{A}}}
\def \Bbar {{\bar{B}}}
\def \Cbar {{\bar{C}}}
\def \Dbar {{\bar{D}}}
\def \Ebar {{\bar{E}}}
\def \Fbar {{\bar{F}}}
\def \Gbar {{\bar{G}}}
\def \Hbar {{\bar{H}}}
\def \Ibar {{\bar{I}}}
\def \Jbar {{\bar{J}}}
\def \Kbar {{\bar{K}}}
\def \Lbar {{\bar{L}}}
\def \Mbar {{\bar{M}}}
\def \Nbar {{\bar{N}}}
\def \Obar {{\bar{O}}}
\def \Pbar {{\bar{P}}}
\def \Qbar {{\bar{Q}}}
\def \Rbar {{\bar{R}}}
\def \Sbar {{\bar{S}}}
\def \Tbar {{\bar{T}}}
\def \Ubar {{\bar{U}}}
\def \Vbar {{\bar{V}}}
\def \Wbar {{\bar{W}}}
\def \Xbar {{\bar{X}}}
\def \Ybar {{\bar{Y}}}
\def \Zbar {{\bar{Z}}}

\def \vecahat {\hat{\vecXX{a}}}
\def \vecbhat {\hat{\vecXX{b}}}
\def \vecchat {\hat{\vecXX{c}}}
\def \vecdhat {\hat{\vecXX{d}}}
\def \vecehat {\hat{\vecXX{e}}}
\def \vecfhat {\hat{\vecXX{f}}}
\def \vecghat {\hat{\vecXX{g}}}
\def \vechhat {\hat{\vecXX{h}}}
\def \vecihat {\hat{\vecXX{i}}}
\def \vecjhat {\hat{\vecXX{j}}}
\def \veckhat {\hat{\vecXX{k}}}
\def \veclhat {\hat{\vecXX{l}}}
\def \vecmhat {\hat{\vecXX{m}}}
\def \vecnhat {\hat{\vecXX{n}}}
\def \vecohat {\hat{\vecXX{o}}}
\def \vecphat {\hat{\vecXX{p}}}
\def \vecqhat {\hat{\vecXX{q}}}
\def \vecrhat {\hat{\vecXX{r}}}
\def \vecshat {\hat{\vecXX{s}}}
\def \vecthat {\hat{\vecXX{t}}}
\def \vecuhat {\hat{\vecXX{u}}}
\def \vecvhat {\hat{\vecXX{v}}}
\def \vecwhat {\hat{\vecXX{w}}}
\def \vecxhat {\hat{\vecXX{x}}}
\def \vecyhat {\hat{\vecXX{y}}}
\def \veczhat {\hat{\vecXX{z}}}
\def \vecalphahat {\hat{\vecXX{\alpha}}}
\def \vecbetahat {\hat{\vecXX{\beta}}}

\def \vecabar {\bar{\vecXX{a}}}
\def \vecbbar {\bar{\vecXX{b}}}
\def \veccbar {\bar{\vecXX{c}}}
\def \vecdbar {\bar{\vecXX{d}}}
\def \vecebar {\bar{\vecXX{e}}}
\def \vecfbar {\bar{\vecXX{f}}}
\def \vecgbar {\bar{\vecXX{g}}}
\def \vechbar {\bar{\vecXX{h}}}
\def \vecibar {\bar{\vecXX{i}}}
\def \vecjbar {\bar{\vecXX{j}}}
\def \veckbar {\bar{\vecXX{k}}}
\def \veclbar {\bar{\vecXX{l}}}
\def \vecmbar {\bar{\vecXX{m}}}
\def \vecnbar {\bar{\vecXX{n}}}
\def \vecobar {\bar{\vecXX{o}}}
\def \vecpbar {\bar{\vecXX{p}}}
\def \vecqbar {\bar{\vecXX{q}}}
\def \vecrbar {\bar{\vecXX{r}}}
\def \vecsbar {\bar{\vecXX{s}}}
\def \vectbar {\bar{\vecXX{t}}}
\def \vecubar {\bar{\vecXX{u}}}
\def \vecvbar {\bar{\vecXX{v}}}
\def \vecwbar {\bar{\vecXX{w}}}
\def \vecxbar {\bar{\vecXX{x}}}
\def \vecybar {\bar{\vecXX{y}}}
\def \veczbar {\bar{\vecXX{z}}}

\def \matA {{\matxx{A}}}
\def \matB {{\matxx{B}}}
\def \matC {{\matxx{C}}}
\def \matD {{\matxx{D}}}
\def \matE {{\matxx{E}}}
\def \matF {{\matxx{F}}}
\def \matG {{\matxx{G}}}
\def \matH {{\matxx{H}}}
\def \matI {{\matxx{I}}}
\def \matJ {{\matxx{J}}}
\def \matK {{\matxx{K}}}
\def \matL {{\matxx{L}}}
\def \matM {{\matxx{M}}}
\def \matN {{\matxx{N}}}
\def \matO {{\matxx{O}}}
\def \matP {{\matxx{P}}}
\def \matQ {{\matxx{Q}}}
\def \matR {{\matxx{R}}}
\def \matS {{\matxx{S}}}
\def \matT {{\matxx{T}}}
\def \matU {{\matxx{U}}}
\def \matV {{\matxx{V}}}
\def \matW {{\matxx{W}}}
\def \matX {{\matxx{X}}}
\def \matY {{\matxx{Y}}}
\def \matZ {{\matxx{Z}}}

\def \matnought {{\matxx{0}}}

\def \matSigma  {{\matxx{\Sigma}}}
\def \matLambda {{\matxx{\Lambda}}}

\def \matAhat {\hat{\matxx{A}}}
\def \matBhat {\hat{\matxx{B}}}
\def \matChat {\hat{\matxx{C}}}
\def \matDhat {\hat{\matxx{D}}}
\def \matEhat {\hat{\matxx{E}}}
\def \matFhat {\hat{\matxx{F}}}
\def \matGhat {\hat{\matxx{G}}}
\def \matHhat {\hat{\matxx{H}}}
\def \matIhat {\hat{\matxx{I}}}
\def \matJhat {\hat{\matxx{J}}}
\def \matKhat {\hat{\matxx{K}}}
\def \matLhat {\hat{\matxx{L}}}
\def \matMhat {\hat{\matxx{M}}}
\def \matNhat {\hat{\matxx{N}}}
\def \matOhat {\hat{\matxx{O}}}
\def \matPhat {\hat{\matxx{P}}}
\def \matQhat {\hat{\matxx{Q}}}
\def \matRhat {\hat{\matxx{R}}}
\def \matShat {\hat{\matxx{S}}}
\def \matThat {\hat{\matxx{T}}}
\def \matUhat {\hat{\matxx{U}}}
\def \matVhat {\hat{\matxx{V}}}
\def \matWhat {\hat{\matxx{W}}}
\def \matXhat {\hat{\matxx{X}}}
\def \matYhat {\hat{\matxx{Y}}}
\def \matZhat {\hat{\matxx{Z}}}

\def \matAbar {\bar{\matxx{A}}}
\def \matBbar {\bar{\matxx{B}}}
\def \matCbar {\bar{\matxx{C}}}
\def \matDbar {\bar{\matxx{D}}}
\def \matEbar {\bar{\matxx{E}}}
\def \matFbar {\bar{\matxx{F}}}
\def \matGbar {\bar{\matxx{G}}}
\def \matHbar {\bar{\matxx{H}}}
\def \matIbar {\bar{\matxx{I}}}
\def \matJbar {\bar{\matxx{J}}}
\def \matKbar {\bar{\matxx{K}}}
\def \matLbar {\bar{\matxx{L}}}
\def \matMbar {\bar{\matxx{M}}}
\def \matNbar {\bar{\matxx{N}}}
\def \matObar {\bar{\matxx{O}}}
\def \matPbar {\bar{\matxx{P}}}
\def \matQbar {\bar{\matxx{Q}}}
\def \matRbar {\bar{\matxx{R}}}
\def \matSbar {\bar{\matxx{S}}}
\def \matTbar {\bar{\matxx{T}}}
\def \matUbar {\bar{\matxx{U}}}
\def \matVbar {\bar{\matxx{V}}}
\def \matWbar {\bar{\matxx{W}}}
\def \matXbar {\bar{\matxx{X}}}
\def \matYbar {\bar{\matxx{Y}}}
\def \matZbar {\bar{\matxx{Z}}}

\def \vecadot {\dot{\vecXX{a}}}
\def \vecbdot {\dot{\vecXX{b}}}
\def \veccdot {\dot{\vecXX{c}}}
\def \vecddot {\dot{\vecXX{d}}}
\def \vecedot {\dot{\vecXX{e}}}
\def \vecfdot {\dot{\vecXX{f}}}
\def \vecgdot {\dot{\vecXX{g}}}
\def \vechdot {\dot{\vecXX{h}}}
\def \vecidot {\dot{\vecXX{i}}}
\def \vecjdot {\dot{\vecXX{j}}}
\def \veckdot {\dot{\vecXX{k}}}
\def \vecldot {\dot{\vecXX{l}}}
\def \vecmdot {\dot{\vecXX{m}}}
\def \vecndot {\dot{\vecXX{n}}}
\def \vecodot {\dot{\vecXX{o}}}
\def \vecpdot {\dot{\vecXX{p}}}
\def \vecqdot {\dot{\vecXX{q}}}
\def \vecrdot {\dot{\vecXX{r}}}
\def \vecsdot {\dot{\vecXX{s}}}
\def \vectdot {\dot{\vecXX{t}}}
\def \vecudot {\dot{\vecXX{u}}}
\def \vecvdot {\dot{\vecXX{v}}}
\def \vecwdot {\dot{\vecXX{w}}}
\def \vecxdot {\dot{\vecXX{x}}}
\def \vecydot {\dot{\vecXX{y}}}
\def \veczdot {\dot{\vecXX{z}}}

\def \vecth    {{\textbf \Theta}}
\def \vecthdot {\dot{\textbf \Theta}}

\def \Ox {\Omega_x}
\def \Oy {\Omega_y}
\def \Oz {\Omega_z}
\def \meanrdot {\langle\vecrdot_s\rangle}
\def \meanr {\langle\vecr_s\rangle}

\def \curlrdot {{\rm curl}(\vecrdot)}
\def \divrdot  {{\rm div}(\vecrdot)}
\def \defrdot  {{\rm def}(\vecrdot)}

\def \apar {a_\parallel}
\def \aper {a_\perp}
\def \apars {a_\parallel^*}
\def \apers {a_\perp^*}

\def \deg {^{\circ}}

%\def \dt {\delta t}
%\def \Dt {\Delta t}
%
%\def \dx {\delta x}
%\def \Dx {\Delta x}
%
%\def \dy {\delta y}
%\def \Dy {\Delta y}

\def \t {\theta}
\def \tdot {\dot{\theta}}

\newcommand{\thdott}{\mbox{$\dot{\theta}_{t}$}}
\newcommand{\thdotmax}{\mbox{$\dot{\theta}_{pmax}$}}

\newcommand{\thddotmax}{\mbox{$\ddot{\theta}_{pmax}$}}
\newcommand{\mthdotmax}{\mbox{$|\dot{\theta}_{pmax}|$}}
\newcommand{\mthddotmax}{\mbox{$|\ddot{\theta}_{pmax}|$}}
\newcommand{\thti}{\mbox{$\theta_{ti}$}}
\newcommand{\thtzero}{\mbox{$\theta_{to}$}}
\newcommand{\thdottzero}{\mbox{$\dot{\theta}_{to}$}}
\newcommand{\thpzero}{\mbox{$\theta_{po}$}}
\newcommand{\thdotpzero}{\mbox{$\dot{\theta}_{po}$}}
\newcommand{\Tv}{\mbox{$T_v$}}
\newcommand{\Tu}{\mbox{$T_u$}}
\newcommand{\Tc}{\mbox{$T_c$}}
\newcommand{\Td}{\mbox{$T_d$}}


% AND SPECIALS

% A 3-element column vector \vecthree{arg1}{arg2}{arg3}
\newcommand{\vecthree}[3]{\left(\begin{array}{c}#1\\#2\\#3\end{array}\right)}

% A 4-element column vector \vecfour{arg1}{arg2}{arg3}{arg4}
\newcommand{\vecfour}[4]{\left(\begin{array}{c}#1\\#2\\#3\\#4\end{array}\right)}

% A 5-element column vector \vecsix{arg1}{arg2}{arg3}{arg4}{arg5}
\newcommand{\vecfive}[5]{\left(\begin{array}{c}#1\\#2\\#3\\#4\\#5\end{array}\right)}

% A 6-element column vector \vecsix{arg1}{arg2}{arg3}{arg4}{arg5}{arg6}
\newcommand{\vecsix}[6]{\left(\begin{array}{c}#1\\#2\\#3\\#4\\#5\\#6\end{array}\right)}

% A 1-element column vector \vecone{arg1}
\newcommand{\vecone}[1]{\left(\begin{array}{c}#1\end{array}\right)}


% A 2-element column vector \vectwo{arg1}{arg2}
\newcommand{\vectwo}[2]{\left(\begin{array}{c}#1\\#2\end{array}\right)}

% A 3-element column right-justified vector \vecthreeright{arg1}{arg2}{arg3}
\newcommand{\vecthreeright}[3]{\left(\begin{array}{r}#1\\#2\\#3\end{array}\right)}


% A 2-element row vector \rowtwo{arg1}{arg2}
\newcommand{\rowtwo}[2]{\left(\begin{array}{cc}#1&#2\end{array}\right)}

% A 3-element row vector \rowthree{arg1}{arg2}{arg3}
% Trouble is this doesn't go to the right height next to 3*3 matrix
\newcommand{\rowthree}[3]{\left(\begin{array}{ccc}#1&#2&#3\end{array}\right)}

% A 4-element row vector \rowfour{arg1}{arg2}{arg3}{arg4}
\newcommand{\rowfour}[4]{\left(\begin{array}{cccc}#1&#2&#3&#4\end{array}\right)}

% A 5-element row vector
\newcommand{\rowfive}[5]{\left(\begin{array}{cccccc}#1&#2&#3&#4&#5\end{array}\right)}

% A 6-element row vector \rowsix{arg1}{arg2}{arg3}{arg4}{arg5}{arg6}
\newcommand{\rowsix	}[6]{\left(\begin{array}{cccccc}#1&#2&#3&#4&#5&#6\end{array}\right)}

% A 7-element row vector \rowseven{arg1}{arg2}{arg3}{arg4}{arg5}{arg6}{arg7}
\newcommand{\rowseven}[7]{\left(\begin{array}{ccccccc}#1&#2&#3&#4&#5&#6&#7\end{array}\right)}

% A 3*3 matrix \matthree{arg11}{arg12}...{arg33}
\newcommand{\matthree}[9]{\left[\begin{array}{ccc}#1&#2&#3\\#4&#5&#6\\#7&#8&#9\end{array}\right]}

% A 2*3 matrix \mattwothree{arg11}{arg12}...{arg23}
\newcommand{\mattwothree}[6]{\left[\begin{array}{ccc}#1&#2&#3\\#4&#5&#6\end{array}\right]}

% A 2*4 matrix \mattwothree{arg11}{arg12}...{arg24}
\newcommand{\mattwofour}[8]{\left[\begin{array}{cccc}#1&#2&#3&#4\\#5&#6&#7&#8\end{array}\right]}

% A 4*4 matrix \matfour{row1}{row2}{row3}{row4}
% The arguments are rows because we can't have more than 9 arguments
\newcommand{\matfour}[4]{\left[\begin{array}{cccc}#1\\#2\\#3\\#4\end{array}\right]}

% A 3*2 matrix \matthreetwo{arg11}{arg12}...{arg32}
\newcommand{\matthreetwo	}[6]{\left[\begin{array}{cc}#1&#2\\#3&#4\\#5&#6\end{array}\right]}

% A 2*2 matrix \mattwo{arg11}{arg12}...{arg22}
\newcommand{\mattwo}[4]{\left[\begin{array}{cc}#1&#2\\#3&#4\end{array}\right]}

% A 1*1 matrix \matone{arg11}
\newcommand{\matone}[1]{\left[\begin{array}{c}#1\end{array}\right]}

% A 3*3 right-justified matrix \matthreeright{arg11}{arg12}...{arg33}
\newcommand{\matthreeright}[9]{\left[\begin{array}{rrr}#1&#2&#3\\#4&#5&#6\\#7&#8&#9\end{array}\right]}

% A matrix transforming between two reference frames (so M with 2 superscripts)
% Argument is just the supersrcipt we want
\newcommand{\mtrans}[1]{\matxx{M^{#1}}}

% A rotation transforming between two reference frames
% (so R with 2 superscripts)
% Argument is just the supersrcipt we want
\newcommand{\rtrans}[1]{\matxx{R^{#1}}}

% A derivative
\newcommand{\diff}[2]{ \frac{d#1}{d#2} }

% A partial derivative
\newcommand{\pdiff}[2]{ \frac{\partial#1}{\partial#2} }

% A bracketed derivative
\newcommand{\bracdiff}[2]{\left( \frac{d#1}{d#2}      \right)}


% Steve's Commands
\def \inv {^{-1}}
%\def \trans {^{\text{\tiny{T}}}}
\def \trans {^{\top}}
\def \invtrans {^{-\top}}

\newcommand{\bracks}[1]{ \left({#1}\right)}
\newcommand{\bbracks}[1]{ \bigl({#1}\bigr)}
\newcommand{\Bbracks}[1]{ \Bigl({#1}\Bigr)}
\newcommand{\BBbracks}[1]{ \Biggl({#1}\Biggr)}

\newcommand{\braces}[1]{ \left[{#1}\right]}
\newcommand{\bbraces}[1]{ \bigl[{#1}\bigr]}
\newcommand{\Bbraces}[1]{ \Bigl[{#1}\Bigr]}
\newcommand{\BBbraces}[1]{ \Biggl[{#1}\Biggr]}

% Extension to matrix formatting allowing table style specification. eg. [c|cc]

% Andy's note: this command requires that you are including the two packages
% in your document above where you include symbols.tex
%\usepackage{amsmath}
%\usepackage{amssymb}
% Otherwise you'll get build errors from LaTeX!

\makeatletter
\renewcommand*\env@matrix[1][*\c@MaxMatrixCols c]{%
  \hskip -\arraycolsep
  \let\@ifnextchar\new@ifnextchar
  \array{#1}}
\makeatother

\newcommand{\RR}{\mathbb{R}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\GL}[1]{\ensuremath{\mathbf{GL}(#1)}}
\newcommand{\SE}[1]{\ensuremath{\mathbf{SE}(#1)}}
\newcommand{\SU}[1]{\ensuremath{\mathbf{SE}(#1)}}
\newcommand{\SO}[1]{\ensuremath{\mathbf{SO}(#1)}}
\newcommand{\SL}[1]{\ensuremath{\mathbf{SL}(#1)}}

\newcommand{\gl}[1]{\ensuremath{{\mathfrak{gl}(#1)}}}
\newcommand{\su}[1]{\ensuremath{{\mathfrak{se}(#1)}}}
\newcommand{\se}[1]{\ensuremath{{\mathfrak{se}(#1)}}}
\newcommand{\so}[1]{\ensuremath{{\mathfrak{so}(#1)}}}


\newcommand{\norm}[1]{\lVert#1\rVert}

